HierCas: Hierarchical Temporal Graph Attention Networks for Popularity Prediction in Information Cascades

Information cascade popularity prediction is critical for many applications, including but not limited to identifying fake news and accurate recommendations. Traditional feature-based methods heavily rely on handcrafted features, which are domain-specific and lack generalizability to new domains. To address this problem, researchers have turned to neural network-based approaches. However, most existing methods follow a sampling-based modeling approach, potentially losing continuous dynamic information that emerges during the information diffusion process. In this paper, we propose Hierarchical Temporal Graph Attention Networks for cascade popularity prediction (HierCas), which operates on the entire cascade graph by a dynamic graph modeling approach. By leveraging time-aware node embedding, graph attention mechanisms, and hierarchical pooling structures, HierCas effectively captures the popularity trend implicit in the complex cascade. Extensive experiments conducted on two real-world datasets in different scenarios demonstrate that our HierCas significantly outperforms the state-of-the-art approaches. We have released our code at https://github.com/Daisy-zzz/HierCas.

==> chapters/Abstract.tex <==
\begin{abstract}
    Information cascade popularity prediction is critical for many applications, including but not limited to identifying fake news and accurate recommendations. Traditional feature-based methods heavily rely on handcrafted features, which are domain-specific and lack generalizability to new domains. To address this problem, researchers have turned to neural network-based approaches. However, existing methods follow a sampling-based modeling approach, potentially losing continuous dynamic information and structural-temporal dependencies that emerge during the information diffusion process. In this paper, we propose a novel framework called Hierarchical Temporal Graph Attention Networks for cascade popularity prediction (HierCas). Unlike existing methods, HierCas operates on the entire cascade graph by a dynamic graph modeling approach. By leveraging time-aware node embedding, temporal graph attention, and hierarchical pooling structures, HierCas effectively captures the popularity trend implicit in the complex cascade. Extensive experiments conducted on two real‐world datasets in different scenarios demonstrate that our HierCas significantly outperforms the state‐of‐the‐art approaches. We have released our code in \url{https://github.com/Daisy-zzz/HierCas}
\end{abstract}

==> table/ablation.tex <==
\begin{table*}[ht]
    \caption{Ablation results of HierCas on two datasets with different observation times, measured by MSLE, SMAPE (lower is better) and $R^2$ (higher is better). The best results are in \textbf{bold} font, the second-best results are \underline{underlined} and the worst results are \dashuline{underlined dashed}.}
    \label{tab:ablation}
    \centering
    \begin{tabular}{lcccccccccccc}
        \toprule
        \multirow{3}{*}{\textbf{Model}} &  \multicolumn{6}{c}{\textbf{Weibo}} & \multicolumn{6}{c}{\textbf{APS}} \\
        \cmidrule(r){2-7} \cmidrule{8-13}
        & \multicolumn{3}{c}{\textbf{0.5 Hour}} &  \multicolumn{3}{c}{\textbf{1 Hour}} & \multicolumn{3}{c}{\textbf{3 Years}} & \multicolumn{3}{c}{\textbf{5 Years}} \\
        \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10} \cmidrule{11-13}
        & \textbf{MSLE} & \textbf{SMAPE} & $\mathbf{R^2}$ & \textbf{MSLE} & \textbf{SMAPE} & $\mathbf{R^2}$ & \textbf{MSLE} & \textbf{SMAPE} & $\mathbf{R^2}$ & \textbf{MSLE} & \textbf{SMAPE} & $\mathbf{R^2}$ \\
        \midrule
        HierCas-noTime & 2.183 & 0.195 & 0.568 & 2.132 & 0.221 & 0.584 & 1.001 & \dashuline{0.184} & 0.435 & 0.868 & 0.196 & 0.493 \\

        HierCas-noSize & \dashuline{2.399} & 0.202 & \dashuline{0.526} & 2.259 & 0.219 & 0.560 & \dashuline{1.015} & \dashuline{0.184} & \dashuline{0.427} & \dashuline{0.898} & \dashuline{0.197} & \dashuline{0.476} \\
        
        HierCas-meanAgg & 2.386 & \dashuline{0.203} & 0.528 & \dashuline{2.273} & \dashuline{0.227} & \dashuline{0.556} & 0.970 & 0.180 & 0.445 & 0.866 & 0.196 & 0.485 \\
        
        HierCas-noMulti & \underline{1.952} & \underline{0.188} & \underline{0.614} & \underline{1.779} & \underline{0.201} & \underline{0.653} & \underline{0.899} & \underline{0.174} & \underline{0.487} & \underline{0.791} & \underline{0.189} & \underline{0.538} \\

        \midrule
        HierCas & \bm{$1.817$} & \bm{$0.186$} & \bm{$0.633$} & \bm{$1.695$} & \bm{$0.194$} & \bm{$0.672$} & \bm{$0.879$} & \bm{$0.172$} & \bm{$0.497$} & \bm{$0.754$} & \bm{$0.187$} & \bm{$0.551$} \\
        \bottomrule
    \end{tabular}
\end{table*}
